Smart Reply: Automated Response Suggestion for Email

In this paper we propose and investigate a novel end-to-end method for automatically generating short email responses, called Smart Reply. It generates semantically diverse suggestions that can be used as complete email responses with just one tap on mobile. The system is currently used in Inbox by Gmail and is responsible for assisting with 10% of all mobile responses. It is designed to work at very high throughput and process hundreds of millions of messages daily. The system exploits state-of-the-art, large-scale deep learning. We describe the architecture of the system as well as the challenges that we faced while building it, like response diversity and scalability. We also introduce a new method for semantic clustering of user-generated content that requires only a modest amount of explicitly labeled data.

==> system_overview.tex <==
\section{Life of a message}
\label{sec:system}

As described earlier, we break down our overall goal into multiple components---constructing a target response space (described in Section~\ref{sec:response_generation}) and then using it to predict and suggest responses for an incoming email message. Here we give an overview of the end to end prediction system, explain the idea and motivation behind specific parts.


\input{inference_diagram}

Refer to the diagram in Figure~\ref{fig:inference_overview}. When a new email
arrives, we apply the following steps:
\todo{It looks bad because Sec numbers are not in order}

\begin{enumerate}
  \item \textbf{Preprocessing:} This includes sentence
segmentation and tokenization, normalization of the text, removal of
boilerplate text and more. We leave discussion of data and preprocessing details to Section~\ref{sec:data}.  %The details of preprocessing are described in Sec.\ref{sec:data}.

 \item \textbf{Triggering:} We run the triggering model based on feedforward neural
network to decide if we want to generate a Smart Reply for the message.
The details of the triggering model are covered in Sec.~\ref{sec:triggering}.

\item \textbf{Scoring:} The next step is to score all responses from a pre-computed whitelist using
an LSTM-based model. The details of this step can be found in
Sec.~\ref{sec:response_selection}. We describe the system that we used to
generate the whitelist in Sec.~\ref{sec:response_generation}.

\item \textbf{Diversity:} Finally, in Sec.~\ref{sec:diversity} we present the component responsible
for ensuring that our suggestions are diverse.

\end{enumerate}

We describe the details of individual steps in the following sections.

